Darwinian Data Structure Selection

Data structure selection and tuning is laborious but can vastly improve an application's performance and memory footprint. Some data structures share a common interface and enjoy multiple implementations. We call them Darwinian Data Structures (DDS), since we can subject their implementations to survival of the fittest. We introduce ARTEMIS a multi-objective, cloud-based search-based optimisation framework that automatically finds optimal, tuned DDS modulo a test suite, then changes an application to use that DDS. ARTEMIS achieves substantial performance improvements for \emph{every} project in $5$ Java projects from DaCapo benchmark, $8$ popular projects and $30$ uniformly sampled projects from GitHub. For execution time, CPU usage, and memory consumption, ARTEMIS finds at least one solution that improves \emph{all} measures for $86\%$ ($37/43$) of the projects. The median improvement across the best solutions is $4.8\%$, $10.1\%$, $5.1\%$ for runtime, memory and CPU usage. These aggregate results understate ARTEMIS's potential impact. Some of the benchmarks it improves are libraries or utility functions. Two examples are gson, a ubiquitous Java serialization framework, and xalan, Apache's XML transformation tool. ARTEMIS improves gson by $16.5$\%, $1\%$ and $2.2\%$ for memory, runtime, and CPU; ARTEMIS improves xalan's memory consumption by $23.5$\%. \emph{Every} client of these projects will benefit from these performance improvements.

==> dacapo_table.tex <==
\begin{table}[t]
\centering
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
%                                         &        &          &        &              \\ \bottomrule
Dacapo Benchmark                              & \#Star & \#LoC    & \#Test & Coverage(\%) \\ \midrule
\\[-0.95em]
fop                                 & 466    & $11,944$ & 71     & $71.5\%$     \\
\\[-0.95em]
xalan                            & 4,428  & $15,246$ & 232    & $86.9\%$     \\
\\[-0.95em]
avrora                                 & 1,148  & $17,244$ & 5,380   & $91.7\%$     \\
\\[-0.95em]
eclipse                                  & 7,525  & $24,395$ & 1,016  & $94.2\%$     \\
\\[-0.95em]
pmd                                 & 898    & $26,128$ & 1,175  & $90.9\%$     \\
\\[-0.95em]
                               & 539    & $36,513$ & 974    & $90.2\%$     \\
\\[-0.95em]
%jenkinsci/gitlab-plugin                      & 356    & $9,867$  & 122    & $40.5\%$     \\
%jhalterman/modelmapper                       & 482    & $16,530$ & 493    & $67.1\%$     \\
%joel-costigliola/assertj-core                & 812    & $121,284$&        & $\%$        \\
junit-team/junit4                            & 5,642  & $27,820$ & 977    & $89.0\%$     \\
\\[-0.95em]
%neo4j-contrib/graph-collections              & 48     & $13,003$ & 53     & $48.6\%$     \\
%scobal/seyren                                & 800    & $6,993$  & 106    & $54.6\%$     \\
%square/javapoet                              & 2,954  & $7,896$  & 295    & $93.8\%$     \\
twitter/GraphJet                             & 344    & $14,881$ & 94     & $90.7\%$     \\ 
\bottomrule
%uber/phabricator-jenkins-plugin              & 187    & $5,517$  & 192    & $91.3\%$     \\ \bottomrule
\end{tabular}}
\caption{Subject projects studied in this research. \#Star, \#Loc, \#Test, and Coverage(\%) are the number of stars, line of code, number of tests, and the line coverage ratio, respectively. All these subjects are retrieved through GitHub on \nth{11} Jan 2017.}
\label{tb:subjects}
\vspace{-2ex}
\end{table}
% mvn cobertura:cobertura to get the coverage: class level



==> preamble.tex <==
\usepackage{graphicx,color}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{url} % do I need this with hyperref?
\usepackage{multicol}
\usepackage{multirow}
\usepackage{setspace} % for double, 1.5, single spacing etc.
\setstretch{0.99}
\usepackage{xspace}
\usepackage{listings}
\usepackage{ifthen}
\usepackage{verbatim}
\usepackage{float} % defines newfloat used below
\usepackage{microtype}
\usepackage{mathptmx}
\usepackage{stmaryrd} %Additional math symbols.
\usepackage{textcomp}
\usepackage[sort&compress]{natbib} 
\usepackage{todos} % Use \todoset{all=off} to turn off todos in a paper.
\usepackage{fixltx2e} 
\usepackage{booktabs}
\usepackage{fancyhdr}


% These two let you use multibyte utf-8 characters, e.g. 03bb - λ 
\usepackage[mathletters]{ucs}
\usepackage[utf8x]{inputenc}
\usepackage{wasysym}	% Defines \cent, \currency, \brokenvert

% hyperref redefines a number of macros, so it should be last.  Empirically,
% doing so eliminates compiler warnings.
\usepackage[bookmarks, colorlinks, citecolor=green, urlcolor=blue,
			filecolor=blue, linkcolor=blue]{hyperref}
% According to the hyperref readme, algorithm must follow hyperref
\usepackage[noend]{algorithmic} % may not be installed
\usepackage{algorithm}


% required for combined latex/pdf xfig figures
\DeclareGraphicsRule{.pdftex}{pdf}{.pdftex}{} 


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~



\newfloat{Protocol}{thp}{lop}
\DeclareMathOperator{\cbar}{||} %denotes concurrency in protocol floats.
\newfloat{Program}{thp}{lop}
\newfloat{Procedure}{thp}{lop}

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Theorems, etc.														{{{2
%\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\bigskip}

%\theoremstyle{plain}
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{cor}[thm]{Corollary}

%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}

%\theoremstyle{definition}
%\newtheorem{defn}{Definition}[section]
%\newtheorem{conj}{Conjecture}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Aliases																{{{1
\newcommand{\infinity}{\infty}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Missing unicode chars, other brokenness in ucs/inputenc {{{1
\DeclareUnicodeCharacter{183}{\cdot}						% ·
\DeclareUnicodeCharacter{931}{\ensuremath\Sigma}			% Σ
\DeclareUnicodeCharacter{9001}{\ensuremath\langle}			% 〈
\DeclareUnicodeCharacter{9002}{\ensuremath\rangle}			% 〉
\DeclareUnicodeCharacter{9608}{\ensuremath\blacksquare}		% █
\DeclareUnicodeCharacter{1013}{\in}							% ϵ
\DeclareUnicodeCharacter{8213}{---}							% ―

\renewcommand{\textcent}{\cent}
\renewcommand{\textcurrency}{\currency}
\renewcommand{\textyen}{\yen}
\renewcommand{\textbrokenbar}{\brokenvert}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~




% vim:foldmethod=marker


==> subjects_table.tex <==
\todo{mike, we can remove this table. Just need to write a paragraph were we present the median values of those projects.}
\todo{Actually, it is nice to have a list of subjects, it helps people to replicate the experiments. But the table is too space consuming.}
\begin{table}[tb]
\captionsetup{font=small}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
Uniformly Selected Projects     & \#Star & \#LoC  & \#Test & Coverage(\%) \\ \midrule
apache/commons-validator                     & 52     & $23,520$ & 527    & $95.9\%$     \\
BiBiServ/jobproxy                            & 2      & $2,524$   & 28     & $28.1\%$     \\
bcdev/coastcolour                            & 5      & $11,663$ & 38     & $42.1\%$     \\
%ChinaQuants/Strata                           & 0      & $393,182$& 13187  & $97.1\%$     \\
camunda/camunda-bpm-mockito                  & 8      & $2,857$  & 33     & $31.9\%$     \\
dick-the-deployer/dick-worker                & 0      & $1,348$  & 18     & $66.8\%$     \\
%facebook/jcommon                             & 455    & $32,252$ & 674    & $45.5\%$     \\
fuinorg/event-store-commons                  & 4      & $12,652$ & 208    & $58.2\%$     \\
fcrepo4/fcrepo4                              & 77     & $33,308$ & 640    & $68.5\%$     \\
%GraphWalker/graphwalker-project              & 46     & $112,076$& 376    & $19.4\%$     \\
gabe-alex/HospitalInfectionsMonitoringSystem & 0      & $1,033$  & 1      & $12.5\%$     \\
google/google-http-java-client               & 572    & $20,637$ & 636    & $69.1\%$     \\
%gazbert/bxbot                                & 30     & $ $  &        & $ \%$     \\
HotelsDotCom/plunger                         & 26     & $3,865$  & 175    & $82.8\%$     \\
imagej/imagej-ops                            & 19     & $48,267$ & 792    & $59.6\%$     \\
johnewart/shuzai                             & 0      & $680$    & 8      & $56.4\%$     \\
jenkinsci/confluence-publisher-plugin        & 13     & $24,927$ & 19     & $27.5\%$     \\
kinow/tap-plugin                             & 4      & $2,804$  & 34     & $62.7\%$     \\
linkedin/cleo                                & 512    & $13,922$ & 75     & $55.5\%$     \\
lipeRomani/controle-financeiro-spring-boot   & 0      & $1,058$  & 1      & $9.2\%$      \\
lynchmaniac/poilight                         & 2      & $2,192$  & 35     & $89.3\%$     \\
lsloan/OpenLRS                               & 0      & $5,229$  & 28     & $26.8\%$     \\
mysu/uma                                     & 3      & $1,343$  & 18     & $31.1\%$     \\
%markosbg/debug                               & 0      & $40,941$ & 5      & $14.4\%$     \\
nazaryan/ShipIt                              & 0      & $3,207$  & 61     & $90.7\%$     \\
PEXPlugins/PermissionsEx                     & 356    & $12,956$ & 63     & $35.0\%$     \\
pfichtner/jrunalyzer                         & 8      & $14,962$ & 78     & $18.1\%$     \\
puneetjaiswal/dropwizard                     & 0      & $29,116$ & 873    & $76.5\%$     \\
rayzeng/fqueue                               & 0      & $3,929$  & 10     & $48.9\%$     \\
roby-rodriguez/rubix-verifier                & 0      & $576$    & 3      & $81.0\%$     \\
sannies/mp4parser                            & 832    & $39,272$ & 170    & $48.6\%$     \\
%svn2github/openid4java                       & 4      & $14,504$ & 114    & $55.5\%$     \\
timmolter/XChange                            & 741    & $94,659$ & 588    & $27.1\%$     \\
xored/vertx-typed-rpc                        & 6      & $705$    & 16     & $66.7\%$     \\
zilaiyedaren/zxing                           & 1      & $42,521$ & 378    & $68.3\%$     \\ \bottomrule
%                                             &        &          &        &              \\ \bottomrule
Popular Projects                              & \#Star & \#LoC    & \#Test & Coverage(\%) \\ \midrule
adyliu/jafka                                 & 466    & $11,944$ & 71     & $71.5\%$     \\
%apache/commons-beanutils                     & 69     & $33,422$ & 1,556  & $86.0\%$     \\
%apache/commons-io                            & 313    & $29,267$ & 1,309  & $92.9\%$     \\
%apache/commons-lang                          & 848    & $74,361$ & 3,973  & $96.7\%$     \\
%bitcoinj/bitcoinj                            & 1030   & $83,632$ & 5272   & $84.4\%$     \\
%DataSketches/sketches-core                   & 420    & $40,881$ & 992    & $82.5\%$     \\
%flaxsearch/luwak                             & 247    & $8,246$  & 168    & $84.1\%$     \\
google/auto:value                            & 4,428  & $15,246$ & 232    & $86.9\%$     \\
google/jimfs                                 & 1,148  & $17,244$ & 5,380   & $91.7\%$     \\
google/gson                                  & 7,525  & $24,395$ & 1,016  & $94.2\%$     \\
google/truth                                 & 898    & $26,128$ & 1,175  & $90.9\%$     \\
IDPF/epubcheck                               & 539    & $36,513$ & 974    & $90.2\%$     \\
%jenkinsci/gitlab-plugin                      & 356    & $9,867$  & 122    & $40.5\%$     \\
%jhalterman/modelmapper                       & 482    & $16,530$ & 493    & $67.1\%$     \\
%joel-costigliola/assertj-core                & 812    & $121,284$&        & $\%$        \\
junit-team/junit4                            & 5,642  & $27,820$ & 977    & $89.0\%$     \\
%neo4j-contrib/graph-collections              & 48     & $13,003$ & 53     & $48.6\%$     \\
%scobal/seyren                                & 800    & $6,993$  & 106    & $54.6\%$     \\
%square/javapoet                              & 2,954  & $7,896$  & 295    & $93.8\%$     \\
twitter/GraphJet                             & 344    & $14,881$ & 94     & $90.7\%$     \\ \bottomrule
%uber/phabricator-jenkins-plugin              & 187    & $5,517$  & 192    & $91.3\%$     \\ \bottomrule
\end{tabular}}
\caption{Subject projects studied in this research. \#Star, \#Loc, \#Test, and Coverage(\%) are the number of stars, line of code, number of tests, and the line coverage ratio, respectively. All these subjects are retrieved through GitHub on \nth{11} Jan 2017.}
\label{tb:subjects}
\vspace{-7ex}
\end{table}
% mvn cobertura:cobertura to get the coverage: class level


